A Hybrid Lagrangian-Eulerian Model for the Structural Analysis of Multifield Datasets

Multifields datasets are common in a large number of research and engineering applications of computational science. The effective visualization of the corresponding datasets can facilitate their analysis by elucidating the complex and dynamic interactions that exist between the attributes that describe the physics of the phenomenon. We present in this paper a new hybrid Lagrangian-Eulerian model that extends existing Lagrangian visualization techniques to the analysis of multifields problems. In particular, our approach factors in the entire data space to reveal the structure of multifield datasets, thereby combining both Eulerian and Lagrangian perspectives. We evaluate our technique in the context of several fluid dynamics applications. Our results indicate that our proposed approach is able to characterize important structural features that are missed by existing methods.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sections/flow.tex <==
\section{Hybrid Lagrangian-Eulerian Model in CFD}
\label{sec:le_cfd}
In this section, we present our new model of geometric saliency for flow visualization.
Our approach applies a \textit{Lagrangian lens} based on a vector field to the analysis of an associated scalar field. 
Specifically, this operation can be considered as "lifting" the trajectory from the physical space to the data space created by the associated scalar field.

Figure~\ref{fig:lagrangian_eulerian} illustrates the above Lagrangian-Eulerian concept. 
A pathline is considered as the trajectory in physical space (visualized as the magenta line in figure~\ref{fig:lagrangian_eulerian}). Each point on the trajectory is a vector in the space-time domain. With an associated scalar field, it is possible to get the local scalar values of every point on the trajectory. Therefore, these local scalar values create a new trajectory in scalar domain as the blue line in figure~\ref{fig:lagrangian_eulerian}.

\begin{figure}[ht]
 \centering
 \includegraphics[width=5.0in]{figures/lagrangian_eulerian/lagrangian_eulerian.eps}
 \caption{An illustration of Lagrangian-Eulerian concept.}
 \label{fig:lagrangian_eulerian}
\end{figure}

Compared to the Eulerian structure definition~\cite{ZD:Barakat2012} which only considers the local properties of different fields and the Lagrangian structure definition (FTLE, section~\ref{sec:lagrangian_coherent_structures}) which only focus on the vector fields, our Lagrangian-Eulerian model provides a non-local structure definition which incorporates all fields in a multi-field dataset.


\subsection{Edge Strength Definition}
\label{sec:le_cfd_edge_strength}
The central idea of our approach is a local edge strength measurement that describes the dissimilarity of data space trajectories $\mathscr{S}$s passing through a small neighborhood around a regular location $\mathbf{x}$.
Our hybrid Lagrangian-Eulerian analysis approach comprises the following steps:
\begin{enumerate}
\item A field of space filling data space trajectories is created;
\item The local edge strength is measured through the gradient of this field.
\end{enumerate}

At a given location $\mathbf{x}_{0}$, a pathline $P_{t_{0},\mathbf{x}_{0}}^{T}$ is generated by tracing the particle on $\mathbf{x}_{0}$ in the vector field with a starting time $t_{0}$ and an integration time $T$.
Considering such a pathline $P_{t_{0},\mathbf{x}_{0}}^{T}$ is a trajectory $\mathscr{T}$ in the space-time domain defined by the problem, we create a trajectory $\mathscr{S}$ in data space by assigning the corresponding scalar attribute values on each point $(\mathbf{x}, t)$ of $\mathscr{T}$.
Applying the above process to every location inside the space domain, we define a field in which each location is a data space trajectory.

%In image processing, edge strength is usually measured by the magnitude of the gradient of the underlying scalar or vector field~\cite{ZD:Canny1986}. 
%With data space trajectories, in contrast, directly estimating a spatial gradient is not readily possible. 

Similar to the method presented in chapter~\ref{chapter:edge_detection}, in our approach, the measurement of edge strength in the resulting space filling data space trajectory field is achieved by estimating a function of neighboring trajectories.

For any location $\mathbf{x}$ in the domain of a given dataset, we define our trajectory function by the following equation,
\begin{equation}
\mathscr{S} = A \cdot \mathbf{x} + \mathbf{b}
 \label{eq:trajectory_function}
\end{equation}

Thus, the spatial variations around $\mathbf{x}$ are determined by its Jacobian $J(\mathbf{x}):=\nabla_{\mathbf{x}} \mathscr{S} \equiv A$ and the edge strength is measured as the spectral norm of $J(\mathbf{x})$: 
\begin{equation}
edge(\mathbf{x}):=\sqrt{\lambda_{max}(J(\mathbf{x})^{T}J(\mathbf{x}))}.
\label{eq:le_edge_strength}
\end{equation}



%\subsection{Numerical Approximation}
%\label{sec:le_cfd_numerical_approximation}
%Without loss of generality, we limit our description here to a two-dimensional uniformly spaced setting. 
%Similar constructions are possible in any spatial dimension and on most types of discrete domains.

%Assume a point $\mathbf{x}_{i,j}:=(i\cdot h, j\cdot h)$ with $h > 0$ and $i,j\in \left \{ 0,\cdots,N \right \}$ in our discrete setting. 
%Furthermore, let $M > 0$ an integer defining a time discretization $t^{m}:=\frac{m/M}{T}$ with $m\in\left \{ 0, \cdots, M \right \}$.
%For a pathline $P_{t_{0},\mathbf{x_{i,j}}}^{T}$ generated by tracing the particle on the grid point $\mathbf{x}_{i,j}$ we define the discrete pathline point
%\begin{equation}
%\mathbf{x}^{m} := P_{t_{0},\mathbf{x}_{i,j}}^{T}(t^{m})
%\end{equation}
%as the discrete representation of the pathline using a numerical integration.

%Next, combing the spatial coordinate $\mathbf{x}^{m}$ with time $t_{0} + t^{m}$ we have the discrete trajectory $\mathscr{T}_{t_{0},\mathbf{x}_{i,j}}^{T}$ in space-time domain.
%Scalar attribute values associated to every discrete space-time points $(\mathbf{x}^{m}, t_{0} + t^{m})$ are computed by interpolating the input scalar field and form the discrete trajectory $\mathscr{S}_{t_{0},\mathbf{x}_{i,j}}^{T}$ in scalar domain. 
%In practice, with hundreds scalar values per trajectory on average, each trajectory is a high-dimensional object.
%Therefore, directly estimating the trajectory function is an expensive task. 
%Furthermore, the vector fields of the problem are usually simulated or observed in a particular region of interest.
%Without a suitable velocity defined outside this region, pathline tracer stops tracing particles when they reach the boundary and causes a different in numbers of scalar values among neighboring trajectories.
%In order to estimate the trajectory function in an efficient and robust way, a mapping~\cite{ZD:Brun2004} from high-dimensional trajectories to a fixed number of parameters and low-dimensional Euclidean feature space is performed on each trajectory. 
%A set of moments~\cite{ZD:Wiki} is employed to capture the statistical properties of a trajectory,
%\begin{equation}
%S_{t_{0},\mathbf{x}_{i,j}}^{T} = (\mu_{1}, \mu_{2}, \cdots)^\intercal
%\end{equation}

%where $S_{t_{0},\mathbf{x}_{i,j}}^{T}$ is the parameterization of $\mathscr{S}_{t_{0},\mathbf{x}_{i,j}}^{T}$. 
%Equation~\ref{eq:trajectory_function} is then turns into the following equation,
%\begin{equation}
%S_{t_{0},\mathbf{x}_{i,j}}^{T} = \widetilde{A} \cdot \mathbf{x}_{i,j} + \widetilde{b}.
%\label{eq:trajectory_function_param}
%\end{equation}

%$\widetilde{A}$ and $\widetilde{b}$ in equation~\ref{eq:trajectory_function_param} are estimated by minimizing the follow function
%\begin{equation}
%min_{\widetilde{A},\widetilde{b}}\sum_{\mathbf{m}\in M(\mathbf{x}_{i,j})}^{}\left \|S_{t_{0}, \mathbf{m}}^{T} - (\widetilde{A},\widetilde{b})\begin{pmatrix}\mathbf{m}
%\\ 1
%\end{pmatrix} \right \|^{2}
%\end{equation}
%where $\mathbf{m}\in M(\mathbf{x}_{i,j})$, and $M(\mathbf{x}_{i,j})$ is a union set of $\mathbf{x}_{i,j}$ and its 8-connected neighbors. Then the derivative of $\mathscr{S}_{t_{0}, \mathbf{x}_{i,j}}^{T}$ with respect to $\mathbf{x}_{i,j}$ is approximated as the derivative of $S_{t_{0}, \mathbf{x}_{i,j}}^{T}$,
%\begin{equation}
%\nabla_{\mathbf{x}_{i,j}} \mathscr{S}_{t_{0}, \mathbf{x}_{i,j}}^{T} \approx \nabla_{\mathbf{x}_{i,j}} S_{t_{0}, \mathbf{x}_{i,j}}^{T} = \widetilde{A}.
%\end{equation}

%Replacing the Jacobian in equation~\ref{eq:le_edge_strength}, the edge strength on $\mathbf{x}_{i,j}$ is then approximated as
%\begin{equation}
%edge(\mathbf{x}_{i,j}) \approx \widetilde{edge}(\mathbf{x}_{i,j}) = \sqrt{\lambda_{max}(\widetilde{A}^\intercal \widetilde{A})}.
%\end{equation}


%\begin{figure}[htbp]
% \centering
% \includegraphics[width=\linewidth]{figures/lagrangian_eulerian/parameters.eps}
% \caption[A comparison of edge strength measured using the presented hybrid Lagrangian Eulerian method with different moments during the trajectory parameterization.]{A comparison of edge strength measured using the presented hybrid Lagrangian-Eulerian method with different moments during the trajectory parameterization. (a) Backward FTLE computed from \textit{Boussinesq Flow} dataset with $t_{0}=3.0$ and $T=2.0$; (b)-(e) edge strength measured by the presented approach using up to $1st$, $2nd$, $3rd$, and $5th$ moments during the trajectory parameterization.}
% \label{fig:parameters}
%\end{figure}

%Figure~\ref{fig:parameters} compares a backward FTLE field computed from \textit{Boussinesq Flow} (Section~\ref{res:boussinesq_flow}) using $t_{0}=3.0$ and $T=2.0$ with the edge strength fields measured by the presented approach with different sets of moments during the trajectory parameterization.
%A set with higher order moments not only is hard to estimate but also presents false structures (highlighted by cyan arrows). In our system, we use the first moment (mean) and the second central moment (variance) to map trajectories to the feature space. 


%\subsection{Implementation}
%\label{sec:le_cfd_implementation}

%In our hybrid Lagrangian-Eulerian approach, the computation of the edge strength measurement for a given problem is built on a large number of scalar domain trajectories. 
%Meanwhile, each scalar domain trajectory requires an individual pathline.
%Even for a small data set, tracing pathlines requires a significant computational effort. 
%In addition, a super-sampling is often necessary to reveal important coherent structures of a given problem, which further increases the computational cost of our approach.

%As we mentioned in section~\ref{sec:le_cfd_edge_strength}, our approach consists of two steps, scalar domain trajectories creation and edge strength measurement.
%In each step, the computation is independent among different point in the discrete setting. 
%Thus, we address this problem by paralleling the computation on a multi-core processor architecture.
%To compare the performance of our hybrid Lagrangian-Eulerian approach with finite-time Lyapunov exponent (FTLE)~\cite{ZD:Haller2001} method, the running time of both method were recorded on a machine with an Intel i7-970 processor (6 cores / 12 threads) and 12GB memory.

%\begin{table*}[ht]
%\centering
%\caption{Running time of different datasets.}
%\label{tab:running_time}
%\begin{tabular}{|c|c|c|c|}
%\hline
%dataset & \begin{tabular}[c]{@{}c@{}}spatial \\ resolution\end{tabular} & FTLE & Lagrangian-Eulerian \\ \hline
%Boussinesq & $800\times 2400$ & 88 minutes & 90 minutes \\ \hline
%Hurricane \textit{Isabel} & $500\times 500\times 100$ & 18 minutes & 18 minutes \\ \hline
%Delta Wing (right bubble) & $600\times 350\times 400$ & 69 hours & 70 hours \\ \hline
%\end{tabular}
%\end{table*}

%Table~\ref{tab:running_time} summarizes the running time of both methods on different datasets.
%The running time of FTLE method and hybrid Lagrangian-Eulerian approach are close to each other. 
%It is because the computational time spends on pathline / flowmap generation dominates the running time in both cases.


\subsection{Numerical Approximation and Implementation Details}
\label{sec:le_cfd_numerical_implementation}
Without loss of generality, we limit our description here to a two-dimensional uniformly spaced setting. 
Similar constructions are possible in any spatial dimension and on most types of discrete domains.

Assume a point $\mathbf{x}_{i,j}:=(i\cdot h, j\cdot h)$ with $h > 0$ and $i,j\in \left \{ 0,\cdots,N \right \}$ in our discrete setting. 
Furthermore, let $M > 0$ an integer defining a time discretization $t^{m}:=\frac{m/M}{T}$ with $m\in\left \{ 0, \cdots, M \right \}$.
For a pathline $P_{t_{0},\mathbf{x_{i,j}}}^{T}$ generated by tracing the particle on $\mathbf{x}_{i,j}$ we define the discrete pathline point
\begin{equation}
\mathbf{x}^{m} := P_{t_{0},\mathbf{x}_{i,j}}^{T}(t^{m})
\end{equation}
as the discrete representation of the pathline using a numerical integration.

Next, combing the spatial coordinate $\mathbf{x}^{m}$ with time $t_{0} + t^{m}$ we have the discrete trajectory $\mathscr{T}_{t_{0},\mathbf{x}_{i,j}}^{T}$ in space-time domain.
Scalar attribute values associated to every discrete space-time point $(\mathbf{x}^{m}, t_{0} + t^{m})$ are computed by interpolating the input scalar field and form the discrete trajectory $\mathscr{S}_{t_{0},\mathbf{x}_{i,j}}^{T}$ in data space.
Instead of directly estimating the trajectory function of equation~\ref{eq:trajectory_function}, a same strategy presented in chapter~\ref{chapter:edge_detection} is applied here. 
We map each data space trajectory to a fixed number of parameters and low-dimensional Euclidean feature space. 
A set of moments~\cite{ZD:Wiki} is employed to capture the statistical properties of a trajectory,
\begin{equation}
S_{t_{0},\mathbf{x}_{i,j}}^{T} = (\mu_{1}, \mu_{2}, \cdots)^\intercal
\end{equation}
where $S_{t_{0},\mathbf{x}_{i,j}}^{T}$ is the parameterization of $\mathscr{S}_{t_{0},\mathbf{x}_{i,j}}^{T}$. 
Equation~\ref{eq:trajectory_function} is then turned into the following equation,
\begin{equation}
S_{t_{0},\mathbf{x}_{i,j}}^{T} = \widetilde{A} \cdot \mathbf{x}_{i,j} + \widetilde{b}.
\label{eq:trajectory_function_param}
\end{equation}

Thus, the edge strength on $\mathbf{x}_{i,j}$ is approximated as
\begin{equation}
edge(\mathbf{x}_{i,j}) \approx \widetilde{edge}(\mathbf{x}_{i,j}) = \sqrt{\lambda_{max}(\widetilde{A}^\intercal \widetilde{A})}.
\end{equation}

\begin{figure}[htbp]
 \centering
 \includegraphics[width=\linewidth]{figures/lagrangian_eulerian/parameters.eps}
 \caption[A comparison of edge strength measured using the presented hybrid Lagrangian Eulerian method with different moments during the trajectory parameterization.]{A comparison of edge strength measured using the presented hybrid Lagrangian-Eulerian method with different moments during the trajectory parameterization. (a) Backward FTLE computed from \textit{Boussinesq Flow} dataset with $t_{0}=3.0$ and $T=2.0$; (b)-(e) edge strength measured by the presented approach using up to $1st$, $2nd$, $3rd$, and $5th$ moments during the trajectory parameterization.}
 \label{fig:parameters}
\end{figure}

Figure~\ref{fig:parameters} compares a backward FTLE field computed from \textit{Boussinesq Flow} (Section~\ref{res:boussinesq_flow}) using $t_{0}=3.0$ and $T=2.0$ with the edge strength fields measured by the presented approach with different sets of moments during the trajectory parameterization.
A set with higher order moments not only is hard to estimate but also presents false structures (highlighted by cyan arrows). In our system, we use the first moment (mean) and the second central moment (variance) to map trajectories to the feature space. 

We recorded the running time of our hybrid Lagrangian-Eulerian approach and finite-time Lyapunov exponent (FTLE)~\cite{ZD:Haller2001} method on a machine with an Intel i7-970 processor (6 cores / 12 threads) and 12GB memory to study the performance of both methods.

\begin{table*}[ht]
\centering
\caption{Running time of different datasets.}
\label{tab:running_time}
\begin{tabular}{|c|c|c|c|}
\hline
dataset & \begin{tabular}[c]{@{}c@{}}spatial \\ resolution\end{tabular} & FTLE & Lagrangian-Eulerian \\ \hline
Boussinesq & $800\times 2400$ & 88 minutes & 90 minutes \\ \hline
Hurricane \textit{Isabel} & $500\times 500\times 100$ & 18 minutes & 18 minutes \\ \hline
Delta Wing (right bubble) & $600\times 350\times 400$ & 69 hours & 70 hours \\ \hline
\end{tabular}
\end{table*}

Table~\ref{tab:running_time} summarizes the running time of both methods on different datasets.
The running time of FTLE method and hybrid Lagrangian-Eulerian approach are close to each other. 
It is because the computational time spends on pathline / flowmap generation dominates the running time in both cases.


\subsection{Results}
\label{sec:le_cfd_results}
We evaluated our method with a number of multi-field datasets from analytic and real-world CFD problems.

\subsubsection{Boussinesq Flow}
The Boussinesq flow used here was simulated using the example provided in Gerris Flow Solver~\cite{ZD:Popinet2004} by the author. 
The simulation uses the classical Boussinesq approximation, in which the conservation of mass (section~\ref{sec:navier_stokes_equations}) is replaced by the conservation of volume (zero divergence), to generate the turbulent vortex behavior in the physical domain $Space \times Time = [-0.5, 0.5] \times [-0.5, 2.5] \times [0.0, 10.0]$. 
With this approximation, fluid heated by some objects, e.g. the heated cylinder in this case, reduces the mass. 
Thus, it moves upward by the buoyancy effect and creates the turbulence~\cite{ZD:Wilcox1998}. 
This simulation result contains a 2D unsteady velocity field as well as an associated temperature field of every time frame.

\label{res:boussinesq_flow}
\begin{figure}[!htbp]
 \centering
 \includegraphics[width=6.0in]{figures/lagrangian_eulerian/boussinesq_comp_2.eps}
 \caption[Salient structures characterized in \textit{Boussinesq flow} dataset using the hybrid Lagrangian-Eulerian method.]{Salient structures characterized in \textit{Boussinesq flow} dataset using the hybrid Lagrangian-Eulerian method. (a) three backward FTLE fields computed with different starting time $t_{0}=2.75$, $t_{0}=3.00$, and $t_{0}=3.25$; (b) ridge lines extracted from those FTLE fields; (c) three edge strength fields measured by the presented approach with a same setting as (a); (d) ridge lines extracted from edge strength fields, color coded by the shortest Euclidean distance to FTLE ridges.}
 \label{fig:boussinesq_flow}
\end{figure}

We applied both the FTLE method and the hybrid Lagrangian-Eulerian approach on this dataset and compared them through the similarity of ridge lines extracted from the resulting scalar fields.
Given two ridge lines $C_{i}={\mathbf{c}_{i}^{1}, \cdots, \mathbf{c}_{i}^{m}}$ and $C_{j}={\mathbf{c}_{j}^{1}, \cdots, \mathbf{c}_{j}^{n}}$ that are represented by polylines with $m$ and $n$ vertices respectively, we define the dissimilarity metric $d_{ij}$ as the distance from $C_{i}$ to $C_{j}$,
\begin{equation}
d_{ij}=\frac{1}{m+n}\left [ \sum_{k=1}^{m}dist(\mathbf{c}_{i}^{k}, C_{j})+\sum_{k=1}^{n}dist(\mathbf{c}_{j}^{k}, C_{i}) \right ]
\end{equation}
where the function $dist(\mathbf{c}_{i}^{k},C_{j})$ returns the shortest Euclidean distance from the vertex $\mathbf{c}_{i}^{k}$ to the piecewise linear curve $C_{j}$.
Instead of finding the maximal value in the union set of $\left \{ dist(\mathbf{c}_{i}^{k}, C_{j}):k\in\left \{ 1,\cdots,m \right \} \right \}$ and $\left \{ dist(\mathbf{c}_{j}^{k}, C_{i}):k\in\left \{ 1,\cdots,n \right \} \right \}$ used in Hausdorff distance metric~\cite{ZD:Huttenlocher1993}, our metric uses the mean value of the same union set.

Figure~\ref{fig:boussinesq_flow} (a) illustrates three backward FTLE fields computed with different starting time $t_{0}=2.75$, $t_{0}=3.00$, and $t_{0}=3.25$. 
Figure~\ref{fig:boussinesq_flow} (b) shows ridge lines extracted from those FTLE fields using Marching Ridge method (section~\ref{sec:marching_ridges}). 
In figure~\ref{fig:boussinesq_flow} (c), three edge strength fields were measured with the same setting as figure~\ref{fig:boussinesq_flow} (a) by the presented hybrid Lagrangian-Eulerian approach. 
We colored each vertex of ridge lines extracted from our edge strength measurement based on the shortest Euclidean distance to FTLE ridges in figure~\ref{fig:boussinesq_flow} (d).
The distances from edge strength ridges to FTLE ridges of the above three results are $7\mathrm{e}{-5}$, $5\mathrm{e}{-5}$, and $6\mathrm{e}{-5}$ and all of them are far less than the distance between neighboring points in our discrete setting ($h=5\mathrm{e}{-4}$).
The comparison on the Boussinesq flow dataset shows in some simple cases, structures characterized by our hybrid Lagrangian-Eulerian approach coincide with the LCS characterized from an FTLE measure.


\subsubsection{Hurricane Isabel}
The \textit{Hurricane Isabel} is the benchmark dataset of IEEE 2004 Visualization Design Contest. 
This dataset was generated by the National Center for Atmospheric Research in the United States to simulate the \textit{hurricane Isabel} in a large region of the West Atlantic in September 2003.
It consists of $13$ variables including a vector field which is the wind speed and $12$ scalar properties such as temperature, pressure, and precipitation for $48$ time frames ($1$ simulated hour between time steps).
The spatial dimension of the dataset is $500\times 500\times 100$ at each time frame.

The hurricane eye is the most recognizable feature and is considered as the focus of a hurricane.
One major goal was to study the path and the structure of the hurricane eye.
A hurricane eye is the center point about which the rest of the storm rotates and where the lowest pressure is found in the hurricane.
The wind will increase its magnitude and converge towards the hurricane eye.
Before reaching the eye, the \textit{Coriolis force} deflects the wind slightly away from it and quickly drops the wind magnitude, causing the wind to rotate around the center of the hurricane, which is named as the hurricane eye wall.
Thus, tracking and analyzing the hurricane eye wall provides an effective way to study the path and the structure of the hurricane eye. 

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=4.0in]{figures/lagrangian_eulerian/hurricane_isabel_ftle_le.eps}
 \caption[Salient structures characterized in \textit{Hurricane Isabel} dataset using the hybrid Lagrangian-Eulerian method.]{Salient structures characterized in \textit{Hurricane Isabel} dataset using the hybrid Lagrangian-Eulerian method. (a) a slice of the pressure volume; (b) Canny edge detection result; (c) FTLE result; (d) hybrid Lagrangian-Eulerian approach result.}
 \label{fig:hurricane_isabel_slice}
\end{figure}

Figure~\ref{fig:hurricane_isabel_slice} (a) shows a slice of the pressure volume. 
The low pressure region (the black spot) on this image indicates the hurricane eye. 
One way to characterize the hurricane eye wall is applying an edge detection method, e.g. Canny edge detector~\cite{ZD:Canny1986}, on the pressure volume as shown in figure~\ref{fig:hurricane_isabel_slice} (b).
However, the noise near the hurricane eye in the pressure volume results in low quality edges.
Because of the convergence and divergence behavior of the wind around the hurricane eye, the Lagrangian method is another way to capture the geometric structure of the hurricane eye wall. 
However, the nearby rainbands and other structures of the hurricane make it difficult to distinguish the hurricane eye wall from other structures detected inside this dataset.
Figure~\ref{fig:hurricane_isabel_slice} (c) illustrates the same slice of the forward FTLE volume computed with integration time $T=2$ hours as figure~\ref{fig:hurricane_isabel_slice} (a).
Using the pressure as the scalar field, and with a same integration time as the FTLE method, our hybrid Lagrangian-Eulerian approach is able to generate a clear and smooth hurricane eye wall result (figure~\ref{fig:hurricane_isabel_slice} (d)).

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=6.0in]{figures/lagrangian_eulerian/hurricane_isabel_eye_track.eps}
 \caption[Tracking the hurricane eye wall in \textit{Hurricane Isabel} dataset.]{Tracking the hurricane eye wall in \textit{Hurricane Isabel} dataset.}
 \label{fig:hurricane_isabel_eye_track}
\end{figure}

Figure~\ref{fig:hurricane_isabel_eye_track} visualizes the edge strength measured by the proposed approach using cutting plane and volume rendering. It is clear that with our approach, one can easily track and analyze the hurricane eye wall in this dataset. 

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=6.0in]{figures/lagrangian_eulerian/hurricane_isabel_result.eps}
 \caption[\textit{Hurricane Isabel} results.]{\textit{Hurricane Isabel} results.}
 \label{fig:hurricane_isabel_result}
\end{figure}

Figure~\ref{fig:hurricane_isabel_result} shows the ridge surfaces extracted from the edge strength volume measured by our hybrid Lagrangian-Eulerian approach.
The resulting ridge surfaces successfully capture the structure of the hurricane eye wall in this dataset.


\subsubsection{Delta Wing}
The so-called Delta Wing dataset is a CFD simulation that is designed to study the transient flow above
a delta wing at low speeds and increasing angle of attack.
The major goal of the simulation was to investigate the cause of the vortex breakdown of the primary vortices.
One velocity field and four scalar attribute fields are included in this dataset.

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=5.0in]{figures/lagrangian_eulerian/delta_wing_ftle_le.eps}
 \caption[A comparison of FTLE and hybrid Lagrangian-Eulerian method in \textit{Delta wing} dataset.]{A comparison of FTLE and hybrid Lagrangian-Eulerian method in \textit{Delta wing} dataset. (a) One slice of the FTLE field computed from this dataset; (b) and (d) closed-up of FTLE field in both vortex breakdown bubbles; (c) and (e) edge strength measured by the presented hybrid Lagrangian-Euleiran approach of both vortex breakdown bubbles.}
 \label{fig:delta_wing_ftle_le}
\end{figure}

Two asymmetric vortex breakdown bubbles, a chaotic one on the left side and a stable one the right side, have already been visualized using stream surfaces in previous studies~\cite{ZD:Tricoche2004,ZD:Garth2005}.
In the Lagrangian method, e.g. FTLE, the main challenge in characterizing LCS of the vortex breakdown bubble is a noisy FTLE field caused by the complexity of the flow near the edge of the delta wing.
Figure~\ref{fig:delta_wing_ftle_le} (a) shows a slice of the backward FTLE field computed from this dataset.
The detailed FTLE fields in regions of both vortex breakdown bubbles of two primary vortices are shown in figure~\ref{fig:delta_wing_ftle_le} (b) and (d).
The unexpected structures at those regions, especially the ones near the outer layer of both vortex breakdown bubbles, make it difficult to extract smooth and meaningful LCS.

\begin{figure}[!htbp]
 \centering
 \includegraphics[width=6.0in]{figures/lagrangian_eulerian/delta_wing_result_right.eps}
 \caption[The right vortex breakdown bubble result.]{The right vortex breakdown bubble result. (a) and (b) volume rendering of the edge strength volume; (c)-(f) ridge surfaces characterized from the same edge strength volume, rendered with opacity and different cutting planes.}
 \label{fig:delta_wing_right_bubble}
\end{figure}

Using the SA viscosity, which is computed from Spalart-Allmaras model~\cite{ZD:Spalart1992}, as the associated scalar field in the presented hybrid Lagrangian-Eulerian approach, our edge strength measurement generates a clear result and captures coherent structures of both vortex breakdown bubbles (figure~\ref{fig:delta_wing_ftle_le} (c) and (e)). 
The resulting edge strength volume of the right vortex breakdown bubble are illustrated in figure~\ref{fig:delta_wing_right_bubble} using volume rendering and ridge surfaces.






==> sections/hardi.tex <==
\section{Hybrid Lagrangian-Eulerian Model in HARDI}
\label{sec:le_hardi}
In this section, we describe a new Lagrangian-Eulerian framework that utilizes two existing methods, namely super-resolution track-weighted imaging~\cite{ZD:Calamante2012} and anisotropy creases~\cite{ZD:Kindlmann2006,ZD:Kindlmann2007}, to visualize and analyze HARDI datasets.

\subsection{Hybrid Lagrangian-Eulerian Framework}
\label{sec:le_hardi_framework}
Before we introduce our hybrid Lagrangian-Eulerian framework for HARDI visualization,
we briefly revisit the concept of super-resolution track-weighted imaging and anisotropy creases.

\subsubsection{Super-resolution Track-weighted Imaging}
Super-resolution track-weighted imaging is a technique that creates a scalar field with higher spatial resolution using whole-brain fiber tracks. 
Particularly, the value of the created scalar field is made dependent on a user specific property of the fiber tracks or their spatial coordinates. 

Let $\{\mathcal{T}_{i}\}, i\in1,\cdots,n$ be the result of whole-brain fiber tracking. 
Each fiber track $\mathcal{T}_{i}$ in this tractogram is computed with a maximum length $l_{max}$ from a diffusion weighted MRI dataset with an acquired voxel size of $nx_{a}\times ny_{a}\times nz_{a}$ $mm^{3}$. 
A number of geometrical properties, such as length, mean curvature and torsion, can be assigned to $\mathcal{T}_{i}$. 
Alternatively, one can assign to $\mathcal{T}_{i}$ a property $p$ of an associated scalar field over its spatial coordinates, such as the mean of a tensor property along the fiber track (e.g. the mean fractional anisotropy (FA) and the average mean diffusivity (MD) discussed in section~\ref{sec:medical_imaging_dti}, as well as the mean generalized fractional anisotropy (GFA)~\cite{ZD:Tuch2004}, along the fiber track). 
This alternative approach is referred as the track-wise statistic. 
In this way, one can link an associated scalar property to $\mathcal{T}_{i}$. 

Assume one would like to reconstruct a new scalar field with a voxel size of $nx_{r}\times ny_{r}\times nz_{r}$ $mm^{3}$ using these linked scalar properties. 
Typically the voxel size of the reconstruct field is smaller than the acquired one, which will lead to the super-resolution nature of the track-weighted imaging technique. 

For a voxel $\mathbf{x}$, one can calculate the mean value of the linked property for each fiber track traversing this voxel:
\begin{equation}
m_{p}\left ( \mathbf{x} \right )=\frac{1}{k\left ( \mathbf{x} \right )}\sum_{i=1}^{k\left ( \mathbf{x} \right )}p_{i},
\end{equation}
where index $i$ indicates the $i$th fiber track traversing the voxel $\mathbf{x}$, and the total number of fiber tracks traversing the voxel $\mathbf{x}$ is given by $k(\mathbf{x})$. 
In this way, a scalar field can be generated by assigning to each voxel the value $m_{p}$. 
Since this scalar field is reconstructed from a tractography result and the fiber tracks provide the additional intra-voxel information, it is able to reveal the features at a sub-voxel level inside a diffusion weighted MRI dataset. 
Figure~\ref{fig:le_hardi_super_resolution} illustrates the super-resolution track-weighted imaging technique.

\begin{figure}[ht]
 \centering
 \includegraphics[width=\linewidth]{figures/lagrangian_eulerian/super_resolution.eps}
 \caption[An illustration of the super-resolution track-weighted technique.]{An illustration of the super-resolution track-weighted technique. (a) Zoomed region in an axial FA map (see inset for location); two elements of the super-resolution grid are highlighted by the blue and yellow pixels. (b) Zoomed area in the neighborhood of the blue grid element, with the tensor lines traversing the grid element overlaid; this location corresponds to an area with a single fiber population (corpus callosum). (c) Zoomed area in the neighborhood of the yellow grid element, with the tensor lines traversing the grid element overlaid; this location corresponds to an area with three fiber populations. The color-coding of the tensor lines is the standard RGB convention (red: left/right, green: anterior/posterior, blue: inferior/superior). (d) Generated super-resolution track-weight image. (from~\cite{ZD:Calamante2012}) }
 \label{fig:le_hardi_super_resolution}
\end{figure}

\subsubsection{Anisotropy Creases}
Anisotropy creases are defined as local extremal of tensor anisotropy. Based on the description in section~\ref{sec:ridges_and_valleys} , anisotropy creases (ridges and valleys) are formed by the points where the gradient of tensor anisotropy is orthogonal to one or more eigenvectors of its Hessian. 

In the method presented by Kindlmann et al.~\cite{ZD:Kindlmann2007}, instead of using a full scale-space extraction of anisotropy creases, it uses a fixed scale Gaussian kernel as a pre-process. The preliminary results suggest that anisotropy ridges coincide with the interiors of white matter fiber tracts, while the anisotropy valleys delineate the boundaries between different fiber tracts that are adjacent but distinctly oriented (e.g. the boundaries between corpus callosum and the cingulum bundles).

Figure~\ref{fig:le_hardi_anisotropy_creases} demonstrates the anisotropy creases in a synthetic dataset. The dataset contains two adjacent fiber bundles which are orthogonal to each other. The anisotropy ridges (red and green surfaces) correctly model the skeleton of these two fiber bundles, while the anisotropy valleys (white surface) captures the interface between them.

\begin{figure}[ht]
 \centering
 \includegraphics[width=\linewidth]{figures/lagrangian_eulerian/anisotropy_creases.eps}
 \caption[Demonstration of anisotropy creases in a synthetic dataset.]{Demonstration of anisotropy creases in a synthetic dataset. The tractography of the two fiber bundles in (a) is color-coded by the usual RGB (major eigenvector). The lower FA between the fiber bundles is highlighted in (b). In (c), the red and green ridge surfaces correctly model the shape of fiber bundles, and the white valley surface captures the interface between them. (from~\cite{ZD:Kindlmann2007})}
 \label{fig:le_hardi_anisotropy_creases}
\end{figure}

\bigskip
\begin{figure}[ht]
 \centering
 \includegraphics[width=\linewidth]{figures/lagrangian_eulerian/hardi_framework.eps}
 \caption[Hybrid Lagrangian-Eulerian HARDI visualization framework.]{Hybrid Lagrangian-Eulerian HARDI visualization framework.}
 \label{fig:le_hardi_framework}
\end{figure}

Figure~\ref{fig:le_hardi_framework} illustrates our hybrid Lagrangian-Eulerian framework for HARDI visualization. 
First, a large number of fiber tracts are generated from the input  HARDI dataset by randomly seeding throughout the interested region(e.g. the white matter of human brain) using iFOD2 fiber tracking method~\cite{ZD:Tournier2010}. 
A generalized fractional anisotropy (GFA) field is also measured from the input HARDI dataset. 
Then, a super-resolution track-weighted field is generated by the fiber tracts and the GFA field created in the previous step. 
Finally, the geometrical structures are characterized as crease surfaces of the super-resolution track-weighted field. 
Since we are interested in the geometrical boundaries of different fiber bundles in this chapter, we employ the anisotropy valleys to characterize sub-voxel features from a super-resolution track-weighted anisotropy field.



\subsection{Results}
\label{sec:le_hardi_results}
We use the public IIT human brain HARDI template~\cite{ZD:Zhang2011} to demonstrate the result obtained by the hybrid Lagrangian-Eulerian framework presented in this section. 
The spatial resolution of the template is $182\times 218\times 182$ with an acquired voxel size of $1.0\times 1.0\times 1.0$ $mm^{3}$. 
This dataset contains a field describing the per-voxel fiber orientation distribution function (fODF) using spherical harmonics up to $6$th order as well as a GFA field.

Figure~\ref{fig:le_hardi_result} presents our results of two regions of interest from the IIT template. 
The first column visualizes the GFA images of these regions. 
The second column shows the reconstructed super-resolution track-weighted images. 
These super-resolution track-weighted images are generated using software MRtrix3~\cite{ZD:Mrtrix} with a reconstruction voxel size of $0.25\times 0.25\times 0.25$ $mm^{3}$ ($64$ times larger than the acquired resolution). 
Comparing the first two columns, the super-resolution track-weight images delineate the substructures in human brain and provide the necessary information used in the later anisotropy creases technique. 
The third column visualizes the valley strength computed from images in the second column using the valley definition described in section~\ref{sec:height_ridge}. 
The last column demonstrates the super-resolution track-weighted images augmented with valley lines. 
These valley lines successfully characterize the boundaries of the highlighted anatomical structures.

\begin{sidewaysfigure}[ht]
 \centering
 \includegraphics[width=7.0in]{figures/lagrangian_eulerian/hardi_result.eps}
 \caption[Anisotropy creases results in human brain HARDI dataset.]{Anisotropy creases results in human brain HARDI dataset. The first column: GFA images of these regions; the second column: reconstructed super-resolution track-weighted images; the third column: valley strength computed from images in the second column; the last column: characterized valley lines. cc: \textit{corpus callosum}; cg: \textit{cingulum}; icp: \textit{inferior cerebellar peduncle}; mcp: \textit{middle cerebellar peduncle}; pcr: \textit{posterior region of corona radiata}; scp: \textit{superior cerebellar peduncle}; scr: \textit{superior region of internal capsule}; sfo: \textit{superior fronto-occipital fasciculus}; slf: \textit{superior longitudinal fasciculus}; *: \textit{short-range association fibers}; **: \textit{vertical occipital fasciculus}.}
 \label{fig:le_hardi_result}
\end{sidewaysfigure}

In figure~\ref{fig:le_hardi_comp}, we compare the results obtained by this hybrid Lagrangian-Eulerian framework and the results achieved by the edge detection method described in chapter~\ref{chapter:edge_detection} (major differences are highlighted by yellow ellipses). 
Our hybrid Lagrangian-Eulerian framework generates a cleaner result and allows focusing on the most important anatomical structures. 

\begin{figure}[ht]
 \centering
 \includegraphics[width=5.0in]{figures/lagrangian_eulerian/le_hardi_comp.eps}
 \caption[A comparison of the results obtained by hybrid Lagrangian-Eulerian framework and edge detection method described in chapter~\ref{chapter:edge_detection}.]{A comparison of the results obtained by hybrid Lagrangian-Eulerian framework and edge detection method described in chapter~\ref{chapter:edge_detection}. Last row shows the edge strength measured by the edge detection method described in chapter~\ref{chapter:edge_detection} and the characterized edges.}
 \label{fig:le_hardi_comp}
\end{figure}

==> sections/lagrangian_eulerian.tex <==
\chapter{HYBRID LAGRANGIAN-EULERIAN MODEL}
\label{chapter:lagrangian_eulerian}

\input{chapters/lagrangian_eulerian/introduction.tex}

\input{chapters/lagrangian_eulerian/flow.tex}

\input{chapters/lagrangian_eulerian/hardi.tex}

==> sections/structure.tex <==
\section{Structure Extraction}
\label{sec:structure}
